Indicative Summarization of Long Discussions

Online forums encourage the exchange and discussion of different stances on many topics. Not only do they provide an opportunity to present one's own arguments, but may also gather a broad cross-section of others' arguments. However, the resulting long discussions are difficult to overview. This paper presents a novel unsupervised approach using large language models (LLMs) to generating indicative summaries for long discussions that basically serve as tables of contents. Our approach first clusters argument sentences, generates cluster labels as abstractive summaries, and classifies the generated cluster labels into argumentation frames resulting in a two-level summary. Based on an extensively optimized prompt engineering approach, we evaluate 19~LLMs for generative cluster labeling and frame classification. To evaluate the usefulness of our indicative summaries, we conduct a purpose-driven user study via a new visual interface called Discussion Explorer: It shows that our proposed indicative summaries serve as a convenient navigation tool to explore long discussions.

==> table-automatic-eval-cluster-labeling.tex <==
\begin{table*}[t]
\centering
\small
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{lccccccccc}
\toprule
\textbf{Model} & \multicolumn{3}{c}{\textbf{\ttfamily Reference}} & \multicolumn{3}{c}{\textbf{\ttfamily {GPT3.5}}} & \multicolumn{3}{c}{\textbf{Length}} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
 & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{Min} &\textbf{Max} & \textbf{Mean} \\
\midrule
\textbf{\ttfamily{Alpaca-7B}} & 0.20 & 0.15 & 0.17 & 0.31 & 0.28 & 0.29 & 3 & 21 & 7.9 \\
\textbf{\ttfamily{Baize-13B}} & 0.17 & 0.15 & 0.16 & 0.33 & 0.32 & 0.32 & 1 & 39 & 8.5  \\
\textbf{\ttfamily{Baize-7B}} & 0.22 & 0.19 & 0.20 & 0.38 & 0.38 & 0.38 & 2 & 46 & 10.7 \\
\textbf{\ttfamily{BLOOM}} & 0.18 & 0.09 & 0.13 & 0.27 & 0.22 & 0.24 & 1 & 37 & 8.0 \\
\textbf{\ttfamily{Falcon-40B}} & 0.12 & 0.09 & 0.10 & 0.17 & 0.17 & 0.17 & 1 & 57 & 9.6 \\
\textbf{\ttfamily{Falcon-40B-Inst.}} & 0.22 & 0.18 & 0.20 & 0.34 & 0.32 & 0.33 & 2 & 33 & 9.3 \\
\textbf{\ttfamily{ChatGPT}} & 0.23 & 0.24 & 0.23 & 0.39 & 0.43 & 0.41 & 3 & 34 & 11.1 \\
\textbf{\ttfamily{GPT4}} & 0.21 & 0.19 & 0.20 & 0.37 & 0.36 & 0.37 & 4 & 18 & 7.5 \\
\textbf{\ttfamily{GPT-NeoX}} & 0.20 & 0.07 & 0.13 & 0.27 & 0.19 & 0.23 & 1 & 34 & 7.4 \\
\textbf{\ttfamily{LLaMA-30B}} & 0.12 & 0.06 & 0.08 & 0.19 & 0.17 & 0.17 &1 & 46 & 9.6 \\
\textbf{\ttfamily{LLaMA-CoT}} & 0.24 & 0.21 & 0.22 & 0.41 & 0.39 & 0.40 & 3 & 29 & 8.4 \\
\textbf{\ttfamily{LLaMA-65B}} & 0.08 & 0.02 & 0.05 & 0.14 & 0.14 & 0.14 & 1 & 46 & 10.3 \\
\textbf{\ttfamily{OASST}} & 0.22 & 0.21 & 0.21 & 0.39 & 0.40 & 0.40 & 3 & 31 & 10.2 \\
\textbf{\ttfamily{OPT}} & 0.17 & 0.09 & 0.13 & 0.24 & 0.20 & 0.22 & 1 & 30 & 8.3 \\
\textbf{\ttfamily{Pythia}} & 0.19 & 0.13 & 0.16 & 0.31 & 0.27 & 0.29 & 2 & 34 & 7.7 \\
\textbf{\ttfamily{T0}} & 0.27 & 0.00 & 0.12 & 0.36 & 0.12 & 0.22 & 1 & 18 & 3.1 \\
\textbf{\ttfamily{GPT3.5}} & 0.23 & 0.06 & 0.14 & 0.49 & 0.31 & 0.40 & 3 & 27 & 9.4 \\
\textbf{\ttfamily{Vicuna-13B}} & 0.21 & 0.21 & 0.21 & 0.36 & 0.39 & 0.37 & 3 & 39 & 11.9 \\
\textbf{\ttfamily{Vicuna-7B}} & 0.20 & 0.19 & 0.19 & 0.34 & 0.37 & 0.35 & 2 & 24 & 11.5 \\
\bottomrule
\end{tabular}
\caption{Complete results of automatic evaluation for the cluster labeling task of all 19 LLMs. We compared them against the manually annotated reference and \textbf{\ttfamily{GPT3.5}}, the best model from our manual evaluation. Also shown are the statistics of the length of the generated cluster labels (in number of tokens).}
\label{tab:automatic-eval-cluster-labeling}
\end{table*}

==> table-best-prompts-clustering.tex <==
\begin{table}[t]
\centering
\small
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{1.2pt}
\begin{tabular}{lp{0.8\columnwidth}}
\toprule
\textbf{Model} & \textbf{Prompt} \\ 
\midrule
T0    & Read the following context and answer the question.\newline Context: \{\emph{text}\} \newline Question: What is the title of the discussion? \newline Answer:  \\                               
\end{tabular}
\caption{Best prompts for each model for generative cluster labeling}
\label{tab:best-prompts-cluster-labeling}
\end{table}

==> table-cluster-label-lengths.tex <==
\begin{table*}[t]
\centering
\small
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{lccc}
\toprule
\textbf{Model} & \textbf{Mean length} & \textbf{Min length} & \textbf{Max length} \\
\midrule
\textbf{\ttfamily{Alpaca-7B}} & 7.9 & 3 & 21 \\
\textbf{\ttfamily{Baize-13B}} & 8.5 & 1 & 39 \\
\textbf{\ttfamily{Baize-7B}} & 10.7 & 2 & 46 \\
\textbf{\ttfamily{BLOOM}} & 8.0 & 1 & 37 \\
\textbf{\ttfamily{Falcon-40B}} & 9.6 & 1 & 57 \\
\textbf{\ttfamily{Falcon-40B-Instruct}} & 9.3 & 2 & 33 \\
\textbf{\ttfamily{GPT-3.5-Turbo}} & 11.1 & 3 & 34 \\
\textbf{\ttfamily{GPT-4}} & 7.5 & 4 & 18 \\
\textbf{\ttfamily{GPT-NeoX}} & 7.4 & 1 & 34 \\
\textbf{\ttfamily{Llama-30B}} & 9.6 & 1 & 46 \\
\textbf{\ttfamily{Llama-30B-SuperCOT}} & 8.4 & 3 & 29 \\
\textbf{\ttfamily{Llama-65B}} & 10.3 & 1 & 46 \\
\textbf{\ttfamily{OASST}} & 10.2 & 3 & 31 \\
\textbf{\ttfamily{OPT-66B}} & 8.3 & 1 & 30 \\
\textbf{\ttfamily{Pythia}} & 7.7 & 2 & 34 \\
\textbf{\ttfamily{T0++}} & 3.1 & 1 & 18 \\
\textbf{\ttfamily{Text-Davinci-003}} & 4.2 & 1 & 13 \\
\textbf{\ttfamily{Text-Davinci-003 (original)}} & 9.4 & 3 & 27 \\
\textbf{\ttfamily{Vicuna-13B}} & 11.9 & 3 & 39 \\
\textbf{\ttfamily{Vicuna-7B}} & 11.5 & 2 & 42 \\
\bottomrule
\end{tabular}
\caption{Lengths of cluster labels generated by the models.}
\label{tab:cluster-label-lengths}
\end{table*}

==> table-models-cluster-labeling.tex <==
\begin{table}[t]
\centering
\small
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}lcp{0.52\columnwidth}@{}}
\toprule
\textbf{Model}    & \textbf{Variants} & \textbf{Description}         \\ 
\midrule
\textbf{\ttfamily{T0}}       & --  & Encoder-decoder model trained on datasets transformed as task-specific prompts. \\
\textbf{\ttfamily{BLOOM}}    & --   & A 176B parameter autoregressive model for prompt-based text completion across multiple languages.              \\
\textbf{\ttfamily{GPT-NeoX}} & 20B & GPT-3 open-source alternative.             \\
\textbf{\ttfamily{OPT}}      & 66B & Autoregressive model with similar performance to GPT-3 albeit with efficient practices for data collection and training.             \\
\textbf{\ttfamily{GPT3.5}}   & text-davinci-003 & Instruction-following LLM that outperforms GPT-3, exclusively available via OpenAI API.%
\footnote{https://platform.openai.com/docs/models/gpt-3-5} \\ 
\bottomrule
\end{tabular}
\caption{List of LLMs investigated for generative cluster labeling. Additional details are provided in Appendix~\ref{sec:appendix-clustering-models}.}
\label{tab:models-cluster-labeling}
\end{table}

==> table-models-frame-assignment.tex <==
\begin{table}[t]
\centering
\small
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{1.2pt}
\begin{tabular}{lcp{0.51\columnwidth}}
\toprule
\textbf{Model}                  & \textbf{Variants}   & \textbf{Description}  \\ 
\midrule
\multicolumn{3}{c}{\colorbox{blue!60!black}{\textcolor{white}{\ttfamily{Direct Instruction}}}} \\
\midrule
\textbf{\ttfamily{LLaMA-CoT}}   &  --           & LLaMA-30B model finetuned on chain-of-thought and logical deduction examples \cite{si:2023}.          \\
\textbf{\ttfamily{Alpaca}}      &  7B           & LLaMA-7B model finetuned on 52K examples of self-instructed instruction-following responses \cite{wang:2022}.              \\
\textbf{\ttfamily{OASST}}       &  --           & LLaMA-30B model finetuned on the OpenAssistant Conversations dataset \cite{koepf:2023} using reinforcement learning.             \\
\textbf{\ttfamily{Pythia}}      &  12B          & A suite of LLMs trained on public data to study the impact of training and scaling on various model properties.\\
\textbf{\ttfamily{GPT*}}        &               & Comprised of OpenAI models including \textbf{\ttfamily{GPT3.5}}(\emph{text-davinci-003}), \textbf{\ttfamily{ChatGPT}}(\emph{gpt-3.5-turbo}), and \textbf{\ttfamily{GPT4}}.              \\
\midrule
\multicolumn{3}{c}{\colorbox{green!40!black}{\textcolor{white}{\ttfamily{Dialogue Instruction}}}} \\
\midrule
\textbf{\ttfamily{LLaMA}}       & 30B, 65B           & A suite of open-source LLMs from Meta AI trained on public datasets.              \\
\textbf{\ttfamily{Vicuna}}      & 7B, 13B          &  LLaMA models finetuned on user-shared conversations collected from ShareGPT.%
\footnote{\url{https://sharegpt.com/}}             \\
\textbf{\ttfamily{Baize}}       & 7B, 13B           & Open-source chat model trained on 100k dialogues generated by allowing ChatGPT (GPT 3.5-turbo) to converse with itself.             \\
\textbf{\ttfamily{Falcon}}      & 40B, 40B-Instruct           & Trained on the RefinedWeb corpus \cite{penedo:2023}, derived through extensive filtering and deduplication of publicly available web data.              \\
\bottomrule
\end{tabular}
\caption{List of LLMs investigated for zero-/few-shot frame assignment. Additional details are provided in Appendix~\ref{sec:appendix-frame-assignment-models}.}
\label{tab:models-frame-assignment}
\end{table}
